State-Space Model Inspired Multiple-Input Multiple-Output Spiking Neurons

In spiking neural networks (SNNs), the main unit of information processing is the neuron with an internal state. The internal state generates an output spike based on its component associated with the membrane potential. This spike is then communicated to other neurons in the network. Here, we propose a general multiple-input multiple-output (MIMO) spiking neuron model that goes beyond this traditional single-input single-output (SISO) model in the SNN literature. Our proposed framework is based on interpreting the neurons as state-space models (SSMs) with linear state evolutions and non-linear spiking activation functions. We illustrate the trade-offs among various parameters of the proposed SSM-inspired neuron model, such as the number of hidden neuron states, the number of input and output channels, including single-input multiple-output (SIMO) and multiple-input single-output (MISO) models. We show that for SNNs with a small number of neurons with large internal state spaces, significant performance gains may be obtained by increasing the number of output channels of a neuron. In particular, a network with spiking neurons with multiple-output channels may achieve the same level of accuracy with the baseline with the continuous-valued communications on the same reference network architecture.

==> code_excerpt.tex <==
%-----------MATLAB CODE -----
% creates a symmetric matrix real valued matrix A using the DFT matrix
N=8; %even


% eig_x : known frequency spectrum (written with the convention first
% non-negative axis 
% and then negative axis)
f_dc=rand(1,1); % trainable real-valued parameter
f_pos= randn(N/2-1,1)+sqrt(-1)*randn(N/2-1,1); % trainable complex-valued parameters
f_pos_last =randn(1,1); % trainable real-valued parameter
eig_x = [f_dc; 
        f_pos; 
        f_pos_last;
        conj(f_pos(end:-1:1,1))]

% dft matrix 
U= dftmtx(N)/sqrt(N);


Kf=diag(eig_x)  % "freq" domain

A=U*Kf*U';  % " time" domain

norm(imag(A)) % should be close to zero if we were able to create a real-valued matrix
norm(real(A)-A) % should be close to zero if we were able to create a real-valued matrix

real(A)
%-----------------------------------------





%-----------Same code but in Python using numpy -----
import numpy as np

# Parameters
N = 8  # Even number

# Create eig_x (frequency spectrum)
f_dc = np.random.rand(1)  # Trainable real-valued parameter
f_pos = np.random.randn(N // 2 - 1) + 1j * np.random.randn(N // 2 - 1)  # Trainable complex-valued parameters
f_pos_last = np.random.randn(1)  # Trainable real-valued parameter

eig_x = np.concatenate([
    f_dc,                     # DC component
    f_pos,                    # Positive frequencies
    f_pos_last,               # Last positive frequency
    np.conj(f_pos[::-1])      # Negative frequencies (Hermitian symmetry)
])

# DFT matrix
U = np.fft.fft(np.eye(N)) / np.sqrt(N)

# Frequency domain diagonal matrix
Kf = np.diag(eig_x)

# Create symmetric matrix A in the time domain
A = U @ Kf @ np.conj(U.T)

# Verify the matrix is real-valued
imag_norm = np.linalg.norm(np.imag(A))  # Should be close to zero
real_diff_norm = np.linalg.norm(np.real(A) - A)  # Should also be close to zero

# Final real-valued matrix
A_real = np.real(A)

# Outputs
print("Norm of imaginary part (should be close to zero):", imag_norm)
print("Norm of difference between real(A) and A (should be close to zero):", real_diff_norm)
print("Real-valued symmetric matrix A:\n", A_real)
%-----------------------------------------




%-----------Part of the main code that does the above in torch -----
import numpy as np
import torch


def one_state_init(N, dt_min=1e-3, dt_max=1e-1):

    # Initialization of continuous time "half N//2" A,B,C
    log_dt = np.random.rand() * (np.log(dt_max) - np.log(dt_min)) + np.log(dt_min)  # Geometrically uniform timescale
    Lambda = -0.5 + 1j * np.pi * np.arange(N//2)  # S4D-Lin initialization
    Lambda_imag = Lambda.imag
    log_Lambda_real = np.log(-Lambda.real)

    # Discretization, obtain discrete time dA,dB,dC for A,B,C respectively. Using bilinear transform
    dt = np.exp(log_dt)
    Lambda = -np.exp(log_Lambda_real) + 1j * Lambda_imag
    dLambda = (1 + dt * Lambda / 2) / (1 - dt * Lambda / 2)

    # Numpy to Pytorch
    dLambda = torch.from_numpy(dLambda).to(dtype=torch.complex64)
    return dLambda


def one_layer_init(N, H):
    """
    :param N: state size
    :param H: hidden size/number of neurons
    """

    # Create for all neurons
    SSM_dLambda = []
    for i in range(H):
        dLambda_i = one_state_init(N=N)
        SSM_dLambda.append(dLambda_i)

    SSM_dLambda = torch.stack(SSM_dLambda)
    return SSM_dLambda


def generate_unitary_matrices(H, N):
    """
    Generate H random unitary matrices of size (N, N).
    Links: https://pytorch.org/docs/stable/generated/torch.linalg.qr.html
    To check if really unitary, you do U.mH @ U, where .mH gives the conjugate
    """
    unitary_matrices = []
    for _ in range(H):

        # SAME DFT MATRIX FOR EACH NEURON
        q = np.fft.fft(np.eye(N)) / np.sqrt(N)
        q = torch.from_numpy(q)

        # IN ANY CASE:
        unitary_matrices.append(q)
    return torch.stack(unitary_matrices)


if __name__ == "__main__":
    N = 8
    H = 16

    Lambda = one_layer_init(N=N, H=H)
    Q = generate_unitary_matrices(N=N, H=H).to(dtype=torch.complex64)


    # Create mixed and real A matrix
    Lambda_extended = torch.cat([Lambda[:, 0:1], # DC component
                                         Lambda[:, 1:], # positive frequencies
                                         Lambda[:, 0:1],  # Nyqvist symmetric component
                                         torch.conj(Lambda[:, 1:].flip(dims=(1,))) # negative frequencies
                                 ],
                                 dim=1)  # Expand from (N/2) to (N) dim,
    N = 2*Lambda.size()[1]  # state dim
    Lambda_extended[:, 0].imag = 0  # Set DC components real
    Lambda_extended[:, N//2].imag = 0  # Set Nyqvist components real
    A = Q.mH @ torch.diag_embed(Lambda_extended) @ Q  # Assume imaginary part is 0
    # A = Q.mH * Lambda_extended.unsqueeze(1) @ Q  # Assume imaginary part is 0

    # Verify the matrix is real-valued
    imag_norm = torch.norm(A.imag)   # Should be close to zero
    real_diff_norm = torch.norm(A.real - A)   # Should also be close to zero

    # Outputs
    print("Norm of imaginary part (should be close to zero):", imag_norm)
    print("Norm of difference between real(A) and A (should be close to zero):", real_diff_norm)


==> errata.tex <==




==> extra_tables.tex <==
\begin{table}[h!]
\centering
\caption{Trade-off between the number of neurons $\Hneurons$  in a hidden layer  and  state dimension of neurons  $\Nstate$ for $\Hneurons \times \Nstate =2048$ where $2$ hidden layered model is used with SISO {\it{signed}}-spiking neurons and \textbf{NON-DIAGONAL} state transition matrix.}
\label{tab:H_vs_N_tradeoff}
\newcolumntype{m}{>{\centering\arraybackslash}p{1.5cm}}
\newcolumntype{l}{>{\centering\arraybackslash}p{2.5cm}}
\begin{tabular}{mml}
 \hline
 $\Hneurons$ & $\Nstate$ & Accuracy \\
 \hline
 1024 & 2 & 82,8$\pm$2,2  \% \\ 
 128 & 16 & 85,6$\pm$1,5 \% \\ 
 64 & 32 &  85,2$\pm$1,6\% \\ 
 32 & 64 &  81,9$\pm$1,9\% \\ 
 16 & 128 & 74,4$\pm$4,5  \% \\ 
 2 & 1024 &  24,4$\pm$7,5\% \\ 
 \hline
\end{tabular}
\end{table}


\begin{table}[h!]
\centering
\caption{Input-Output dimension comparison and trade-off. Neurons with \textbf{NON-DIAGONAL} transition matrix and {\it{signed}}-spiking activation function used.
Architecture used \textbf{$\Hneurons=32, \Nstate=64$}.}
\label{tab:SISO_MIMO_comparison_H32N64}
\newcolumntype{m}{>{\centering\arraybackslash}p{1.2cm}}
\newcolumntype{l}{>{\centering\arraybackslash}p{2.5cm}}
\begin{tabular}{mmml}
 \hline
 Type & Input Dim & Output Dim & Accuracy \\
 \hline
 \multirow{1}{*}{SISO} & 1 & 1 &  83,3$\pm$1,9 \% \\  
    \hline
 \multirow{3}{*}{SIMO} & 1 & 8 & 78,8$\pm$3,1  \% \\ 
                         & 1 & 64 &  85,2$\pm$0,9 \% \\  
                         & 1 & 128 & 85,8$\pm$1,1 \% \\  
    \hline
 \multirow{3}{*}{MISO} & 8 & 1 &  41,2$\pm$5,6 \% \\ 
                         & 64 & 1 & 31,8$\pm$3,4 \% \\  
                         & 128 & 1 & 31,8$\pm$3,4 \% \\  
    \hline
 \multirow{3}{*}{MIMO} & 8 & 8 & 49,9$\pm$5,7 \% \\ 
                         & 64 & 64 &  50,5$\pm$2,0  \% \\  
                         & 128 & 128 & 53,5$\pm$3,5  \% \\  
 \hline
\end{tabular}
\end{table}


\begin{table}[h!]
\centering
\caption{Input-Output dimension comparison and trade-off. Neurons with \textbf{NON-DIAGONAL} transition matrix and {\it{signed}}-spiking activation function used. Architecture used \textbf{$\Hneurons=128, \Nstate=16$}.}
\label{tab:SISO_MIMO_comparison_H128N16}
\newcolumntype{m}{>{\centering\arraybackslash}p{1.2cm}}
\newcolumntype{l}{>{\centering\arraybackslash}p{2.5cm}}
\begin{tabular}{mmml}
 \hline
 Type & Input Dim & Output Dim & Accuracy \\
 \hline
 \multirow{1}{*}{SISO} & 1 & 1 & 86,6$\pm$1,4 \% \\  
    \hline
 \multirow{3}{*}{SIMO} & 1 & 8 & 86,4$\pm$1,5 \% \\ 
                         & 1 & 64 & 87,1$\pm$1,5  \% \\  
                         & 1 & 128 & 87,3$\pm$1,1  \% \\  
    \hline
 \multirow{3}{*}{MISO} & 8 & 1 & 56,9$\pm$2,7  \% \\ 
                         & 64 & 1 & 43,5$\pm$2,9  \% \\  
                         & 128 & 1 & 46,8$\pm$4,6 \% \\  
    \hline
 \multirow{3}{*}{MIMO} & 8 & 8 &  72,8$\pm$2,2 \% \\ 
                         & 64 & 64 &  67,4$\pm$3,2 \% \\  
                         & 128 & 128 &  68,9$\pm$3.5\% \\  
 \hline
\end{tabular}
\end{table}

==> presentation_notes.tex <==

Sanja notes for presentation:
1) "in our setup single output  still gives mixed output so we cannot say that this gain is due to having mixed outputs.  It is the diversity, ie, having multiple outputs. Let me know if you disagree."
